Learning Optimal Linear Block Transform by Rate Distortion Minimization

Linear block transform coding remains a fundamental component of image and video compression. Although the Discrete Cosine Transform (DCT) is widely employed in all current compression standards, its sub-optimality has sparked ongoing research into discovering more efficient alternative transforms even for fields where it represents a consolidated tool. In this paper, we introduce a novel linear block transform called the Rate Distortion Learned Transform (RDLT), a data-driven transform specifically designed to minimize the rate-distortion (RD) cost when approximating residual blocks. Our approach builds on the latest end-to-end learned compression frameworks, adopting back-propagation and stochastic gradient descent for optimization. However, unlike the nonlinear transforms used in variational autoencoder (VAE)-based methods, the goal is to create a simpler yet optimal linear block transform, ensuring practical integration into existing image and video compression standards. Differently from existing data-driven methods that design transforms based on sample covariance matrices, such as the Karhunen-Lo\`eve Transform (KLT), the proposed RDLT is directly optimized from an RD perspective. Experimental results show that this transform significantly outperforms the DCT or other existing data-driven transforms. Additionally, it is shown that when simulating the integration of our RDLT into a VVC-like image compression framework, the proposed transform brings substantial improvements. All the code used in our experiments has been made publicly available at [1].

==> Figures/Table_BD.tex <==
\begin{table}[]
\centering
\small
\caption{BD-PSNR and BD-Rate comparison with DCT as the anchor.}
\begin{tabular}{@{}ccc@{}}
\toprule
            & BD-PSNR (dB)  & BD-Rate (\%)    \\ \midrule
DCT         & 0             & 0               \\
KLT         & -0.51         & 10.82           \\
SOT         & 0.41          & -7.82           \\
RDLT (Ours) & \textbf{0.68} & \textbf{-12.75} \\ \bottomrule
\end{tabular}
\label{tab:BD_mix}
\end{table}

% \begin{table}[]
% \label{tab:BD_mix}
% \centering
% \small
% \caption{BD-PSNR and BD-Rate comparison with DCT as the anchor.}
% \begin{tabular}{@{}ccc@{}}
% \toprule
%             & BD-PSNR (dB)  & BD-Rate (\%)    \\ \midrule
% DCT         & 0             & 0               \\
% KLT         & -0.83         & 15.62           \\
% SOT         & 0.58          & -9.81           \\
% RDLT (Ours) & \textbf{0.72} & \textbf{-12.16} \\ \bottomrule
% \end{tabular}
% \end{table}

==> Figures/abaltion_RD.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/univ_follow_mix_sub_ablation.jpg}
    \caption{Rate-accuracy comparison for ablation study on transform design choices.}
    \label{fig:RD_ablation}
\end{figure}
